Generating Synthetic Data with Formal Privacy Guarantees: State of the Art and the Road Ahead

Privacy-preserving synthetic data offers a promising solution to harness segregated data in high-stakes domains where information is compartmentalized for regulatory, privacy, or institutional reasons. This survey provides a comprehensive framework for understanding the landscape of privacy-preserving synthetic data, presenting the theoretical foundations of generative models and differential privacy followed by a review of state-of-the-art methods across tabular data, images, and text. Our synthesis of evaluation approaches highlights the fundamental trade-off between utility for down-stream tasks and privacy guarantees, while identifying critical research gaps: the lack of realistic benchmarks representing specialized domains and insufficient empirical evaluations required to contextualise formal guarantees. Through empirical analysis of four leading methods on five real-world datasets from specialized domains, we demonstrate significant performance degradation under realistic privacy constraints ($\epsilon \leq 4$), revealing a substantial gap between results reported on general domain benchmarks and performance on domain-specific data. %Our findings highlight key challenges including unaccounted privacy leakage, insufficient empirical verification of formal guarantees, and a critical deficit of realistic benchmarks. These challenges underscore the need for robust evaluation frameworks, standardized benchmarks for specialized domains, and improved techniques to address the unique requirements of privacy-sensitive fields such that this technology can deliver on its considerable potential.

==> INCFIGS/forest.tex <==
\forestset{
  dir node/.style={
    parent anchor=south west,
    child anchor=west,
    anchor=west,
    inner ysep=-4pt,
    align=left,
    font=\itshape\footnotesize,
  },
  dir tree/.style={
    for tree={
      grow'=0,
      dir node,
      edge path={
        \noexpand\path [draw, \forestoption{edge}] (!u.parent anchor) ++(1em,-0.17em) |- node[fill,inner sep=1.25pt] {} (.child anchor)\forestoption{edge label};
      },
      if n children=0{}{
        font=\bfseries\small,
        delay={
          prepend={[text 1, dir node, phantom, calign with current]}
        }
      },
      fit=band,
      before computing xy={
        l=1.5em,
      }
    },
  }
}

\begin{figure}[!htb]
\begin{framed}
\begin{forest}
  dir tree,
  [Annotation Schema
    [Supporting Fact]
    [Answer Type
        [Paraphrasing - Generated\\
        Span - Unanswerable]
    ]
    [Correctness
        [Debatable - Wrong]
    ]
    [Reasoning
        [Operational
            [Bridge - Comparison - Constraint - Intersection]
        ]
        [Arithmetic
            [Substraction - Addition\\
             Ordering - Counting - Other]
        ]
        [Linguistic
            [Negation - Quantifiers - Conditional\\
            Monotonicity - Con-/Disjunction 
            ]
        ]
        [Temporal]
        [Spatial]
        [Causal]
        [By Exclusion]
        [Retrieval]
    ]
    [Knowledge
        [Factual,
            [Cultural/Historic - (Geo)Political/Legal\\
            Technical/Scientific - Other Domain Specific]
        ]
        [Intuitive]
    ]
    [Linguistic Complexity
        [Lexical Variety
            [Redundancy - Lexical Entailment\\
            Dative - Synonym/Paraphrase\\
            Abbreviation - Symmetry]
        ]
        [Syntactic Variety
            [Nominalisation - Genitive - Voice]
        ]
        [Lexical Ambiguity
            [Restrictivity - Factivity\\
            Coreference - Ellipse/Implicit]
        ]
        [Syntactic Ambiguity
            [Preposition - Listing - Coordination Scope\\
            Relative Clause/Adverbial/Apposition
            ]
        ]
    ]
  ]
\end{forest}
\end{framed}
\caption{The hierarchy of categories in our proposed annotation framework. Abstract higher-level categories are presented in bold while actual annotation features are shown in italics.}
\label{fig:taxonomy}
\end{figure}

==> INCFIGS/table-summary.tex <==

    \begin{tabular}{|p{2cm}|p{4.5cm}|p{4.5cm}|p{4.5cm}|}
    
    \hline
    \textbf{Evaluation Aspect} & \textbf{Tabular Data} & \textbf{Image Data} & \textbf{Text Data} \\
    \hline
    \textbf{Fidelity} &
    \begin{itemize}[leftmargin=*]
        \itemsep0em 
        \item Structural similarity (schema preservation)
        \item Univariate distribution similarity (Jensen-Shannon Divergence, category recovery ratio for categorical; Wasserstein distance for continuous)
        \item Multivariate dependency similarity (correlation matrices)
        \item Global structure \& diversity (propensity score metrics, manifold coverage)
    \end{itemize} &
    \begin{itemize}[leftmargin=*]
        \item Fr\'echet Inception Distance (FID)
        \item Embedding space distributions
        \item Wasserstein distance between means and covariances
    \end{itemize} &
    \begin{itemize}[leftmargin=*]
        \item MAUVE metric (distribution divergence via $k$-means clustering)
        \item KL divergence in embedding space
        \item Distribution of text lengths
    \end{itemize} \\
    \hline
    \textbf{Utility} &
    \begin{itemize}[leftmargin=*]
        \item Performance on specific downstream tasks
        \item Classification/regression accuracy
        \item Model training on synthetic data, evaluation on real data
        \item Preservation of performance rankings across methods
    \end{itemize} &
    \begin{itemize}[leftmargin=*]
        \item Classification accuracy
        \item Performance in domain-specific tasks
    \end{itemize} &
    \begin{itemize}[leftmargin=*]
        \item Classification accuracy
        \item Language modeling performance (perplexity for decoder models)
        \item Fill-in-the-mask accuracy for encoder models
    \end{itemize} \\
    \hline
    \textbf{Privacy} &
    \begin{itemize}[leftmargin=*]
        \item Formal DP guarantees ($\epsilon$ parameter)
        \item Membership Inference Attacks (MIA)
        \item Shadow-modeling technique
        \item Meta-classifier training
    \end{itemize} &
    \begin{itemize}[leftmargin=*]
        \item Formal DP guarantees
        \item Implementation verification
        \item MIA with various attacker knowledge assumptions
    \end{itemize} &
    \begin{itemize}[leftmargin=*]
        \item Model-based MIA (attacking models trained on synthetic data)
        \item Formal DP guarantees
        \item Various attacker knowledge assumptions
    \end{itemize} \\
    \hline
    \textbf{Benchmark Datasets} &
    \begin{itemize}[leftmargin=*]
        \item Medical data (e.g., MIMIC-III)
        \item Financial data (e.g., credit card fraud)
        \item Census data
    \end{itemize} &
    \begin{itemize}[leftmargin=*]
        \item CIFAR
        \item MNIST
        \item FashionMNIST
        \item CelebA
    \end{itemize} &
    \begin{itemize}[leftmargin=*]
        \item Sentiment analysis datasets (Yelp, IMDb, Amazon reviews)
        \item PubMed abstracts
        \item Topic modeling datasets
    \end{itemize} \\
    \hline
    \textbf{Key Trade-offs} & \multicolumn{3}{p{13.5cm}|}{
    \begin{itemize}[leftmargin=*]
        \item Utility vs. privacy trade-off: As privacy bounds tighten (lower $\epsilon$), more noise is added, degrading data quality
        \item Formal guarantees vs. empirical privacy: Formal DP provides worst-case bounds while MIA measures practical leakage
        \item Standardized benchmarks are lacking across all modalities
    \end{itemize}
    } \\
    \hline
    \end{tabular}

